Teacher-Student Training for Debiasing: General Permutation Debiasing for Large Language Models

Large Language Models (LLMs) have demonstrated impressive zero-shot capabilities and versatility in NLP tasks, however they sometimes fail to maintain crucial invariances for specific tasks. One example is permutation sensitivity, where LLMs' outputs may significantly vary depending on the order of the input options. While debiasing techniques can mitigate these issues, and yield better performance and reliability, they often come with a high computational cost at inference. This paper addresses this inefficiency at inference time. The aim is to distill the capabilities of a computationally intensive, debiased, teacher model into a more compact student model. We explore two variants of student models: one based on pure distillation, and the other on an error-correction approach for more complex tasks, where the student corrects a single biased decision from the teacher to achieve a debiased output. Our approach is general and can be applied to both black-box and white-box LLMs. Furthermore, we demonstrate that our compact, encoder-only student models can outperform their larger, biased teacher counterparts, achieving better results with significantly fewer parameters.

==> dumping_ground <==
############### was in old theory ####################
% An alternative relaxed measure looks at 
% %
% To quantify this bias, one can consider any two possible permutations $\sigma_1, \sigma_2$ and measure the divergence $\mathcal{D}$ between the resulting distributions:
% %
% \begin{equation*}
%     \label{eq:pairwise-bias}
%     \mathbbm{E}_{\sigma_{j, m}}
%     \left[
%     \mathcal{D}
%     \Big[
%     {\tt P}_{\theta}\left(\cdot | x, o_{\sigma_j(1:K)}\right) ;
%     {\tt P}_{\theta}\left(\cdot | x, o_{\sigma_m(1:K)}\right)
%     \Big]
%     \right]
% \end{equation*}
% %

% to measure the inherent robustness to an invariance, and 


% from \textit{permutation bias}.
% %
% % \subsection{Quantifying Permutation Bias}
% % The options $o_{1:K}$ exist, however the prompt is filled in with a particular implicit ordering of the options. $o_{1:K}$ is the original arbitrary ordering of the set of options, let $M_j(o_{1:K})$ represent a particular ordering of the options. One would want the model to be insensitive to this particular invariance, and the output probabilities to be unaffected by changing the ordering.
% % \begin{equation}
% %     P_{\theta}(y | x_q, x_c, o_{1:K}) = P_{\theta}(y % | x_q, x_c, M_j(o_{1:K})) \quad \forall j
% % \end{equation}
% %

% This is a strict measure of bias in which the model needs to be exactly sensitive to the ordering of the options. An alternative relaxed measure looks at the average probability mass associated with each \textbf{position} $k \in \{1, \dots, K\}$ as opposed to \textbf{option} $o_i$. 
% %
% \begin{equation}
%     {\tt P}_{\sigma}(k|x, o_{1:K}) = \mathbbm{E}_{\sigma_j} \! \left[ {\tt P} \left(k|x, o_{\sigma_j(1:K)}\right) \right]
% \end{equation}
% % \begin{equation}
% %     {\tt P}_{\sigma}(k|x, o_{1:K}) = \mathbbm{E}_{\sigma} \left[{\tt P}_{\theta}\left(o_{\sigma(i)}|x, o_{\sigma(1:K)}\right)\right]
% % \end{equation}
% %
% If this \textit{positional distribution} is non-uniform ${\tt U}(\cdot)$, the natural interpretation is that the underlying LLM has a biased preference for a particular position. Therefore, a measure of \textit{positional bias} can be defined as the divergence between the positional and uniform distribution $\mathcal{D}[{\tt P}_{\sigma}(\cdot|x, o_{1:K}) ; {\tt U}(\cdot)]$.


% % One would expect a uniform distribution over the positions. Any deviation from this would be indicative of a sensitivity to ordering bias. To quantify the level of positional bias, one can consider the distance to a uniform distirbution via total variation,
% % \begin{equation}
% %     bias(x_q, x_c, \theta) = \sum_k | P_{\theta}(k|x_q, x_c, \mathcal{X}_o) - \mathcal{U}(K) |
% % \end{equation}


% % The permutation sensitivity for a particular question $x_q$, context $x_x$ and set of options $o_{1:K}$ can be denoted as:

% % \begin{equation}
% %     \text{bias}(\theta, \mathcal{T}) = \sum_{I\in\mathcal{P} } \sum_{y} || P(y|) - P()||
% % \end{equation}

